A Meta-Complexity Characterization of Quantum Cryptography

We prove the first meta-complexity characterization of a quantum cryptographic primitive. We show that one-way puzzles exist if and only if there is some quantum samplable distribution of binary strings over which it is hard to approximate Kolmogorov complexity. Therefore, we characterize one-way puzzles by the average-case hardness of a uncomputable problem. This brings to the quantum setting a recent line of work that characterizes classical cryptography with the average-case hardness of a meta-complexity problem, initiated by Liu and Pass. Moreover, since the average-case hardness of Kolmogorov complexity over classically polynomial-time samplable distributions characterizes one-way functions, this result poses one-way puzzles as a natural generalization of one-way functions to the quantum setting. Furthermore, our equivalence goes through probability estimation, giving us the additional equivalence that one-way puzzles exist if and only if there is a quantum samplable distribution over which probability estimation is hard. We also observe that the oracle worlds of defined by Kretschmer et. al. rule out any relativizing characterization of one-way puzzles by the hardness of a problem in NP or QMA, which means that it may not be possible with current techniques to characterize one-way puzzles with another meta-complexity problem.

==> formaltest.tex <==
% \newpage
% \section{Lemma 3}

\begin{lemma}\label{lem:firstlem}
    Let $m = \ceil{-\log p_x}$ and $\Pr_{\D \to x'}[p_{x'} \leq 2^{-m}] \geq n^{-c}$.

    Let $k \leq m - 2\log n^c$. Then
    $$\Pr_{h}[\Pr_{\D' \to x}[h(x') = h(x)\text{ and }x'\neq x] \leq 2^{-k-1} n^{-c}] \leq 4n^{-c}$$
    where $h$ is drawn from a $3$-wise independent hash family $\{0,1\}^n \to \{0,1\}^k$.
\end{lemma}

\begin{proof}
    Define $\epsilon = \Pr_{\D \to x'}[p_{x'} \leq 2^{-m}]$.

    Define $\gamma = \Pr_{\D \to x'}[h(x') = h(x)\text{ and }x'\neq x\text{ and }p_{x'} \leq 2^{-m}]$, a random variable in $h$. Define $R_{x'} = p_{x'} \mathds{1}[h(x') = h(x)]$. We have
    $$\gamma = \sum_{x' \neq x:p_{x'} \leq 2^{-m}} R_{x'}$$

    Note that $\E[R_{x'}] = p_{x'}\cdot \Pr[h(x') = h(x)] \leq p_{x'}\cdot 2^{-k}$.

    Furthermore, $\E[R_{x'}^2] = p_{x'}^2 \cdot \Pr_h[h(x') = h(x)] = p_{x'}^2 \cdot 2^{-k}$.

    And so 
    $$\E[\gamma] = \sum_{x' \neq x:p_{x'} \leq 2^{-m}}p_{x'}\cdot \Pr_h[h(x') = h(x)] = 2^{-k} \cdot \Pr_{\D \to x'}[p_{x'} \leq 2^{-m}] = 2^{-k}\cdot \epsilon$$

    By $3$-wise independence of $h$, the $R_{x'}$'s are pairwise independent, so
    $$\Var(\gamma) = \sum_{x' \neq x:p_{x'} \leq 2^{-m}} p_{x'}^2\cdot 2^{-k} \leq \sum_{x' \neq x:p_{x'} \leq 2^{-m}} p_{x'}\cdot 2^{-(m+k)} = 2^{-(m+k)}\cdot \epsilon$$

    Chebyshev inequality then says that
    \begin{equation}
        \begin{split}
            \Pr\left[\gamma \leq 2^{-k}\epsilon - 2^{-k}\epsilon/2\right] \leq \frac{\Var(\gamma)}{(2^{-k}\epsilon/2)^2}\\
            = \frac{4}{\epsilon}2^{-m+k}\cdot 2^{2k}
        \end{split}
    \end{equation}
    And so plugging in $k = m - 2c\log n$ and $\epsilon \leq n^{-c}$, we get
    $$\Pr\left[\gamma \leq 2^{-k-1} n^{-c}\right] \leq 4n^c \cdot 2^{-2c\log n} \leq 4n^{-c}$$
    Since $\Pr_{\D' \to x}[h(x') = h(x)\text{ and }x'\neq x] \geq \gamma$, the theorem follows.
\end{proof}

\begin{lemma}\label{lem:secondlem}
    Let $m = \ceil{-\log p_x}$.

    Then
    $$\Pr_{h}[\Pr_{\D' \to x}[h(x') = h(x)\text{ and }x'\neq x] \geq t\cdot 2^{-k}] \leq t^{-1}$$
    where $h$ is drawn from a $3$-wise independent hash family $\{0,1\}^n \to \{0,1\}^k$.
\end{lemma}

\begin{proof}
    Let $\alpha = \Pr_{\D' \to x}[h(x') = h(x)\text{ and }x'\neq x]$.
    A simple calculation of expectation gives us
    \begin{equation}
        \begin{split}
            \E_h [\alpha] = \sum_{x' \neq x} p_{x'}\cdot 2^{-k}\\
            \leq 2^{-k}
        \end{split}
    \end{equation}
    and so Markov bound says
    $$\Pr[\alpha \geq t\cdot 2^{-k}] \leq t^{-1}$$
    and we are done.
\end{proof}

\begin{lemma}
    Let $m$ be such that $p_x \leq 2^{-m}$ and $\Pr_{\D \to x'}[p_{x'} \leq 2^{-m}] \geq n^{-c}$.

    If $k \leq m - 2c \log n-1$, then
    $$\Pr[P_{k,x} \to x] \leq n^{-c}$$
    If $k \geq m$, then
    $$\Pr[P_{k,x} \to x] \geq \frac{9}{10}$$
\end{lemma}

\begin{proof}
    Define $\alpha = \Pr_{\D' \to x}[h(x') = h(x)\text{ and }x'\neq x]$ a random variable in $h$.

    Let us first consider $k\leq m-2c\log n-1$.~\Cref{lem:firstlem} gives us
    $$\Pr[\alpha \leq n^{-c}\cdot 2^{-k-1}] \leq 4n^{-c}$$
    Let us define $P_{k,h,x}$ to be $P_{k,x}$ conditioned on the hash function being $h$. Note that if $\alpha \geq n^{-c}\cdot 2^{-k-1}$, then
    \begin{equation}
        \begin{split}
            \Pr[P_{k,h,x} \to x] = \frac{p_x}{\alpha + p_x}\\
            \leq \frac{p_x}{n^{-c}\cdot 2^{-k-1} + p_x}\\
            \leq \frac{p_x}{n^{c}\cdot 2^{-m} + p_x}\\
            \leq \frac{p_x}{n^{c}\cdot p_x + p_x}\leq \frac{1}{n^c + 1} \leq n^{-c}
        \end{split}
    \end{equation}
    And so we get that
    $$\Pr[P_{k,x} \to x] \leq \Pr[\alpha \leq n^{-c}\cdot 2^{-k-1}] + n^{-c} = 5n^{-c}$$

    We now consider the case where $k \geq m + 11$. By~\Cref{lem:secondlem}
    $$\Pr_{h}[\alpha \geq t\cdot 2^{-k}] \leq t^{-1}$$
    Furthermore, if $\alpha \leq t\cdot 2^{-k}$, then
    \begin{equation}
        \begin{split}
            \Pr[P_{k,h,x} \to x] = \frac{p_x}{\alpha + p_x}\\
            \geq \frac{p_x}{t\cdot 2^{-k} + p_x}\\
            \geq \frac{p_x}{t\cdot 2^{-10} p_x + p_x}\\
            \geq \frac{1}{t\cdot 2^{-10} + 1}
            \geq \frac{1}{t/1000 + 1}
        \end{split}
    \end{equation}
    Picking $t = 100$, we get 
    \begin{equation}
        \begin{split}
            \Pr\left[P_{k,x} \to x] \geq \Pr[P_{k,h,x} \to x | \Pr_{\D' \to x}[\alpha \leq t\cdot 2^{-k}]\right]\Pr_{\D' \to x}[\alpha \leq t\cdot 2^{-k}]\\
            \geq \frac{99}{100}\frac{1}{1/10 + 1} \geq \frac{99}{100}\frac{10}{11} = \frac{9}{10}
        \end{split}
    \end{equation}
\end{proof}


==> intro.tex <==
\section{Introduction}

What is the minimal natural complexity assumption required for
computational cryptography? Over the last few years a series of works have
attempted to answer this question by giving characterizations of one way
functions (OWFs) via meta-complexity \cite{santhanam2020pseudorandomness,
liu2020one, ilango2021hardness, hirahara2023capturing}. These works have
been motivated by one way functions' centrality. One way functions are
minimal---all classical modern cryptography implies the existence of OWFs,
mostly through trivial reductions. And one way functions are useful---they
can be used to build the many powerful tools of Minicrypt
\cite{impagliazzo1995personal} including commitments, PRGs, and secret key
cryptography. These meta-complexity characterizations have shown that these
powerful tools exists if and only if specific meta-complexity problems are
hard. Liu and Pass showed that they exists if and only if polynomial time
bounded Kolmogorov complexity $\K^{poly}$ is hard on the uniform
distribution \cite{liu2020one} and Ilango, Ren, and Santhanam showed that
they exist if and only if the promise problem $\GapK[s,s+\omega(\log n)]$
is hard on some distribution \cite{ilango2021hardness}. This knowledge has
let us better understand OWFs, the meta-complexity problems that
characterize them, and the relationships between Impagliazzo's worlds. 
\bnote{GapK is unclear. We also need to motivate meta-complexity
    characterisations more (see, e.g., IRS intro). Even
    complexity-theoretic characterisations
    \emph{per se} are not well motivated here -- I think that's how we
    should start. Why characterise primitives? Say what is known classically,
    and why to do it quantumly.
    \\
    The five worlds as
    discussed below is perhaps one other motivation, but it feels a bit
    disconnected as it currently is.
    \\
    We can also talk about:
    \begin{enumerate}
        \item Complexity-theory of OWFs (equivalent to many other
            primitives)
        \item Potential way of trying to connect different quantum
            primitives, or understand their relative powers --
            from the perspective of complexity-theoretic assumptions
            which characterise them.
            Talk about only known consequences being PP != BQP, but
            not known to be sufficient (Kretschmer, our work)
        \item
            Obtaining \emph{natural} problems which characterise a
            cryptographic primitive is important (Levin universal OWF)
        \item In connection with this, talk about why meta-complexity is
            so interesting -- its connections, 'naturality' as a concept,
            etc. etc.
        \item 
            Connection with average-case hardness (here we start touching
            Impagliazzo) -- samplable distributions, etc.
        \item 
            Talk more about QCCC world of One-Way Puzzles, why so
            important.
            Explain more about why it plays a sort of 'OWF role' in it,
            AND talk about how this work establishes this
            more firmly
    \end{enumerate}
}

Impagliazzo's worlds can be seen as 5 different answers to the question ``How much does $\P$ equal or not equal $\NP$?''. Algorithmica is the world corresponding to the simplest answer to the question ``$\P=\NP$!'' This is the world of ultimate computational power, we can build automated theorem provers which can efficiently decide all the open questions we could devise and then collectively retire as theoretical computer scientists; classical computational cryptography would not exist but that would be a small price to pay. Heuristica corresponds to the answer ``we can solve $\NP$ problems with high probability over reasonable distributions''. This is sufficient to rule out cryptography and be usable in many other practical settings, but might not be quite enough to put us all out of work. Pessiland (which Impagliazzo called ``the worst of all possible worlds'') answers the question with there are many hard distributions of $\NP$ problems, but cryptography still does not exist. Minicrypt answers the question with ``$\NP$ is hard enough in practice that we can construct one way functions'' (efficiently computable functions $f$ that are hard to invert) and all the cryptography that comes with them. And Cryptomania answers the question with ``$\NP$ is so hard that we can construct very powerful cryptographic primitives like key exchange and public key encryption''.

One of the major efforts being conducted on the boarder of complexity theory and cryptography is an attempt to collapse these worlds.  

Pessiland (which Impagliazzo called ``the worst of all possible worlds'') particular has been recast as a ``wonderland for learning'' \cite{hirahara2023learning} by examining the meta-complexity impacts of living in a world without OWFs.

However, this focus on OWFs as the minimal assumption for computational cryptography has been complicated by recent work in quantum cryptography. Starting with Ji, Liu, and Song's introduction of pseudorandom states (PRS) \cite{ji2018pseudorandom}, recent work has defined a new suite of quantum cryptographic primitives, most of which appeared to be less powerful than OWFs. Kretschmer formalized this appearance by introducing an oracle world in which PRS (and the many primitives which they imply) exist, but $\BQP=\QCMA$ \cite{Kretschmer21} meaning that no post quantum OWFs are possible. While few formal barriers to equivalences have been shown, it appears likely that these new primitives will end up in a layered hierarchy instead of collapsing into a minicrypt style equivalence class. Currently the two weakest primitives of interest are quantum bit commitments (EFI) \cite{brakerski2022computational, yan2022general} which seem to be minimal for settings with quantum communication, and one way puzzles (OWPuzz) which seem to be minimal in the quantum-computation classical-communication (QCCC) \cite{austrin2022impossibility, chung2024central} setting. The existence of these weaker quantum cryptographic primitives has opened up the possibility of more minimal complexity assumptions for characterizing the existence of computational cryptography. 


This work gives a meta-complexity characterization (which is weaker than $\P \neq \NP$) for the existence of the first of these primitives, the one way puzzle. 

\begin{theorem}
    The following are equivalent:
    \begin{itemize}
        \item One way puzzles exist.
        \item There exists some quantum samplable distribution on which constant factor probability estimation is hard on average.
        \item For some $s = n^{\Omega(1)}$ and $\Delta = \omega(log(n))$ there is a quantum samplable distribution $\D$ over classical strings such that $\GapK[s,s+\Delta]$ is weakly quantumly average-case hard on $\D$.
    \end{itemize}    
\end{theorem}

One way puzzles were introduced by Khurana and Tomer \cite{khurana2024commitments} as an intermediate primitive between Morimae and Yamakawa's one way state generator (OWSG) \cite{morimae2022quantum} and quantum bit commitments, and were studied as an object of independent interest by Chung, Goldin, and Gray \cite{chung2024central}. They fall near the base of the current hierarchy of quantum cryptographic primitives (only EFI is believed to be a weaker primitive) and have several properties desirable for a cryptographic primitive including combiners, a universal construction, and hardness amplification. However they have one feature that seems very strange from a classical perspective, their solutions are not efficiently verifiable.

A OWPuzz is defined by a pair Samp and Ver, where Samp is a quantum poly time algorithm sampling key puzzle pairs (k,s) and Ver is some arbitrary verification function. Correctness requires that $\Pr_{(k,s) \sim Samp}[Ver(k,s) = 1] \geq 1 - \negl$. Security requires that for any poly time quantum adversary $A$, $\Pr[Ver(A(s),s) = 0] \geq 1 - \negl$. The decision by Khurana and Tomer to have verification be inefficient was required by the desire to construct them from OWSGs. To construct a OWPuzz they took the output states of OWSGs and efficiently extracted their classical shadows \cite{huang2020predicting}. However, verifying such a shadow is a statistical process. Chung, Goldin, and Gray decided to generalize the definition further to allow for an arbitrary verification function to overcome ensure correctness when creating a universal OWPuzz. Despite this oddity, one way puzzles can be used to generate pseduo-entropy which allows for both the construction of quantum bit commitments and opens them up to meta-complexity attacks and characterizations.

We also show a barrier to giving further characterizations of OWPuzz. In Kretchmer et al's oracle world OWPuzz exist while $\P = \NP$\cite{KQST23}. In this world, meta-complexity measures whose answers have poly time verifiable witnesses (such as $\K^{poly}$ or MCSP) are easy to compute even in the worst case, and therefore on every distribution. Consequently any characterization of OWPuzz by the hardness of a meta-complexity property must either be non-relativizing or involve a problem (like $\GapK$) whose answers may not have efficiently verifiable witnesses since there is no bound given on the runtime of the generating computation. This shared characteristic of $\GapK$ and OWPuzz of having inefficient verification, seems then to be essential to our characterization.

% Outline:
% -Motivation
% \begin{enumerate}
%     \item IRS/LP shows metacomplexity $\iff$ OWF. Useful because OWF "minimal" for classical cryptography.
%     \item Quantum landscape looks completely different. Many things "below" OWF. EFI minimal for quantum comm. OWPuzz minimal for classical comm.
%     \item Two views: crypto to motivate metacomplexity and metacomplexity to motivate crypto
%     \item Question 1: Are one way puzzles interesting? They are minimal but not useful. Equivalence to hardness of metacomplexity makes them interesting in some sense. They imply quantum sampleable distributions which are hard to estimate. Maybe also hard to learn?
%     \item Question 2: Is there any sense that metacomplexity is hard when P=NP?
% \end{enumerate}


==> introv2.tex <==
\section{Introduction 2nd pass}
Cryptography and complexity theory are two sides of the same coin: computational hardness. Complexity theory categorizes problems by how difficult they are to solve. Cryptography theory shows how hard problems can be used to our advantage. It seems natural that we should expect a deep connection between cryptographic primitives and complexity-theoretic hardness conjectures. 

Some connections do in fact exist. It is easy to observe that if one-way functions exist (OWFs, the most basic cryptographic assumption), then $P\neq NP$ (the most fundamental complexity-theoretic conjecture). Furthermore, there is a long tradition of building cryptographic primitives from the computational hardness of \textit{specific} problems, e.g. factoring, Learning-with-Errors, \dots\todo{citations}. However, these implications only go in a single direction. It would be very nice to have a result along the lines of "cryptography exists if and only if some complexity-theoretic conjecture holds." 

The "holy grail" result of this form\todo{cite metacomplexity talks} would be to show that one-way functions exist if and only if $P\neq NP$. Note that one-way functions are the "central" cryptographic primitive. One way functions are minimal---almost all classical modern cryptography implies the existence of OWFs, mostly through trivial reductions. And one way functions are useful---they can be used to build everything in the crypto-complexity class Minicrypt \cite{impagliazzo1995personal} including commitments, pseudorandom generators, and secret key cryptography. Similarly, $P\neq NP$ is the central conjecture in complexity theory. If it is shown to be false, much of complexity theory becomes trivial\todo{cite PH collapse, P=BPP, ...}. Thus, if the holy grail result is true, then it implies the more general claim that "cryptography is possible if and only if complexity theory is interesting."

For many years, researchers have tried and failed to achieve this holy grail~\cite{FOCS:BogTre03,STOC:AGGM10,TCC:BogBrz15}. However, some progress has come in recent years from a surprising direction, meta-complexity. 

Meta-complexity is the study of computational problems which are themselves about computational complexity. The foremost example of a meta-complexity problem is the question of computing the Kolmogorov complexity of a string $K(x)$, that is the length of the shortest Turing machine outputting that string\todo{cite}. In the past few years, a number of results have shown that the hardness of various meta-complexity problems characterizes the existence of one-way functions\todo{cite}. For the purposes of this work, we will focus on~\cite{ilango2021hardness}, which shows that one-way functions exist if and only if there exists a sampleable distribution on which Kolmogorov complexity is hard to approximate.

However, this focus on OWFs as the minimal assumption for computational cryptography has been complicated by recent work in quantum cryptography. Starting with Ji, Liu, and Song's introduction of pseudorandom states (PRS) \cite{ji2018pseudorandom}, recent work\todo{cite these} has defined a new suite of quantum cryptographic primitives, most of which appeared to be less powerful than OWFs. Kretschmer formalized this by introducing an oracle world in which PRS (and the many primitives which they imply) exist, but $\BQP=\QCMA$ \cite{Kretschmer21} meaning that no post quantum OWFs are possible\footnote{~\cite{STOC:KQST23} similarly shows a classical oracle under which PRSs exist but $P=NP$.}. 

Thus, in the quantum setting, the classical holy grail result is no longer relevant. It is possible that $P=NP$, but useful cryptography exists. This brings up the question

\begin{center}
    \textit{What is the minimal natural complexity assumption required for quantum cryptography?}
\end{center}

To answer this question, the first thing to look at are the minimal primitives for quantum cryptography. Currently the two weakest primitives of interest are quantum bit commitments (EFI) \cite{brakerski2022computational, yan2022general} which seem to be minimal for settings with quantum communication, and one way puzzles (OWPuzz) which seem to be minimal in the quantum-computation classical-communication (QCCC) \cite{STOC:KhuTom24, chung2024central} setting\enote{not sure what the Austrin paper has to do with anything}. One-way puzzles can also be constructed from a number of important quantum output primitives, such as pseudorandom states and one-way state generators~\cite{STOC:KhuTom24, cavalar2023computation}. Notably, the existence of OWPuzz implies that $BQP \neq PP$~\cite{cavalar2023computation}. On the other hand, there are barriers to showing that the existence of EFI implies any conjectures in complexity theory~\cite{STOC:LomMaWri24}.

In this work, we will focus on the seemingly easier question of developing a characterization for one-way puzzles. A one-way puzzle is defined by a quantum sampler algorithm, which samples a puzzle and a corresponding key, as well as an inefficient verification algorithm. The puzzle and key for a OWPuzz must be classical strings. The puzzle should be easy to sample, but hard to solve. That is, sampled puzzle, key pairs should pass verification, but given just the puzzle it should be hard to find a key which verifies. We show that just like with OWFs, OWPuzz can be characterized by the average-case hardness of a meta-complexity problem. 

\begin{theorem}
    The following are equivalent:
    \begin{itemize}
        \item One way puzzles exist.
        \item There exists some quantum samplable distribution on which
            constant factor probability estimation is hard on average.
        \item There is a quantum samplable distribution $\D$ over classical
            strings such that for $\D \to x$ it is hard to decide whether
            $K(x) \leq s$ or $K(x) \geq s + 
            % \omega(\log \secpa)$.
            \omega(\log n)$.
            \bnote{The previous version was not compilling here.}
    \end{itemize}    
\end{theorem}

\paragraph*{Towards bypassing the separation between OWFs and
OWPuzz}Interestingly, the only difference between our hard problem and the
hard problem of~\cite{ilango2021hardness} characterizing OWFs is that our
hardness is over quantum sampleable distributions whereas theirs is over
classically sampleable distributions. This means that if one could somehow
show that hardness of Kolmogorov complexity over quantum and classical
sources are equivalent, then one could also build a OWF from a OWPuzz. Note
that since both our result and the result of~\cite{ilango2021hardness} are
relativizing, such an approach would necessarily use non-relativizing
techniques. However, as Kolmogorov complexity deals directly with Turing
machines, it is fairly amenable to non-relativizing techniques.\enote{move to open Qs?}

\paragraph*{On the importance of one-way puzzles}\enote{I'm not a huge fan of this section. It needs another pass for sure.} One way puzzles were introduced by Khurana and Tomer \cite{khurana2024commitments} as an intermediate primitive between Morimae and Yamakawa's one way state generator (OWSG) \cite{morimae2022quantum} and EFI pairs, and were studied as an object of independent interest by Chung, Goldin, and Gray \cite{chung2024central}. They fall near the base of the current hierarchy of quantum cryptographic primitives (only EFI is believed to be a weaker primitive) and have several properties desirable for a cryptographic primitive including combiners, a universal construction, and hardness amplification. 

Prior work shows that a large number of quantum primitives (pseudorandom states, one-way state generators, and all of QCCC cryptography) can be used to build one-way puzzles~\cite{STOC:KhuTom24,C:ChuGolGra24}. Furthermore, one-way puzzles can be used to build EFI pairs, as well as everything else equivalent to them, such as multi-party computation and quantum bit commitments~\cite{STOC:KhuTom24}. However, one-way puzzles are not useful on their own, and there are barriers to using OWPuzz to build primitives other than EFI pairs~\cite{C:ChuGolGra24}. Thus, it is not immediately clear how important it is to study OWPuzz directly.

One way to view our result is as giving more evidence that OWPuzz are valuable to study as an independent primitive. Even forgetting about OWPuzz, our result gives a complexity theoretic characterization in the following sense. We show that if estimating Kolmogorov complexity is hard, then some important quantum primitives exist (EFI/multi-party computation). Furthermore, if other important quantum primitives exist (pseudorandom states/one-way state generators) then estimating Kolmogorov complexity is hard. However, since hardness of Kolmogorov complexity characterizes OWPuzz specifically, we can also read our result as saying that OWPuzz embody some fundamental aspect of quantum cryptographic hardness.

\paragraph*{Other meta-complexity characterizations are difficult}
Recall that there exists an oracle relative to which OWPuzz exist but $BQP = QMA$. This means that any characterization of OWPuzz by a problem in $QMA$ must by necessity be non-relativizing. However, most meta-complexity characterizations of OWFs \textit{do} relativize.

In particular, other meta-complexity problems known to characterize OWFs can easily be seen to be in $NP$. Examples include the minimum circuit size problem as well as time-bounded Kolmogorov complexity\todo{cite}. Thus,~\cite{Kretschmer21} provides a concrete barrier to showing that variants of these problems characterize OWPuzz. That is, our characterization is the only meta-complexity problem for which current techniques have any hope of proving a characerization of quantum cryptography.

Finally, since our results do relativize, and since there exists an oracle relative to which $P=NP$ but OWPuzz exist, our results also provide a barrier to showing that Kolmogorov complexity estimation can be solved using an $NP$ oracle. This is not surprising, computing Kolmogorov complexity exactly is undecideable\todo{cite}, but this is not an observation we are aware of existing elsewhere.


==> lemma3.tex <==
\section{Proof of Lemma 3}

\begin{lemma}\label{lem:chebtrick}
    $$\Pr_{h,\D\to x}\left[\abs{\Pr_{\D\to x'}[h(x') = h(x)] - \frac{1}{2^k}} \geq t\right] \leq \frac{1}{t^2 2^{k}}$$
\end{lemma}

\begin{proof}
    Define $R_{x'}$ to be the random variable in $h,x$ defined by
    $$R_{x'} = \Pr[\D \to x']\cdot \mathds{1}[h(x') = h(x)]$$

    We can observe that $\Pr_{\D\to x'}[h(x') = h(x)] = \sum_{x'} R_{x'}$. Note also that
    $$\E_{h,x}\left[\sum_{x'} R_{x'}\right] = \sum_{x'} \Pr[\D \to x']\frac{1}{2^k} =\frac{1}{2^k}$$

    As $h$ is a $3$-wise independent hash function, the variables $X_i$ are pairwise independent.

    We have 
    $$\Var(R_{x'}) \leq \E[R_{x'}^2] = \frac{\Pr[\D \to x']^2}{2^{k}} \leq \frac{\Pr[\D \to x']}{2^{k}}$$
    and so
    $$\Var\left(\sum_{x'} R_{x'}\right) \leq \frac{1}{2^{k}}$$

    And so by Chebyshev's inequality,
    $$\Pr_{h,\D\to x}\left[\abs{\Pr_{\D\to x'}[h(x') = h(x)] - \frac{1}{2^k}} \geq t\right] \leq \frac{1}{t^2 2^{k}}$$
\end{proof}

We then proceed to prove
\begin{lemma}[\Cref{claim:approx} restated]
    If $2^{-k} \leq p_x$, then $\Pr[P_{k,x} \to x] \geq \frac{1}{2}$.
    If $2^{-k} \geq 6p_x$, then $\Pr[P_{k,x} \to x] \leq \frac{1}{4}$.
\end{lemma}

\begin{proof}
    Define $P_{k,h,x}$ to be $P_{k,x}$ conditioned on the hash function chosen being $h$.

    We will first consider the case $2^{-k} \leq p_x$. By~\Cref{lem:chebtrick}, we know that
    $$\Pr_{h,\D\to x}\left[\abs{\Pr_{\D\to x'}[h(x') = h(x)] - \frac{1}{2^k}} \geq \frac{1}{2^k}\right] \leq \frac{1}{t^2 2^k}$$
\end{proof}

==> probest.tex <==
% \section{Probability estimation from the inexistence of one-way puzzles}
\section{Probability Estimation from the Nonexistence of One-way Puzzles}

In this section we prove
% our key technical theorem. 
% We will show 
that the non-existence
of one-way puzzles implies algorithms for probability estimation on all
quantum samplable distributions.


\begin{theorem}[Item 2 $\implies$ Item 1]
    \label{thm:owpuzz-probest}
    If one-way puzzles do not exist, 
    then, for any family of quantum
    samplable distributions $\D_{n}$,
    there exists a QPT algorithm that performs probability estimation on
    $\cald$ infinitely often.
    % and for all $d>0$, there exists an
    % algorithm $\cala(x)$ such that
    % $$\Pr_{x\randfrom \mathcal{D}}[p_x\leq \cala(x) \leq 8p_x] \geq 1 - n^{-d}$$
    % infinitely often.
\end{theorem}

The result will follow from the following lemma.
\begin{lemma}
    \label{lemma:probest}
    % % For all $c>0$,
    % Let $c > 0$ 
    % and
    % let $\cald$ be a quantum samplable distribution.
    % For $x \in \blt^n$, let $p_x := \Pr[\cald_n \to x]$.
    % If there do not exist $n^{-c}$-secure distributional one way puzzles,
    % % then for any family of quantum samplable distributions $\D$,
    % then
    % there is an algorithm 
    % % $A(x)$ 
    % $\cala$
    % % which estimates 
    % % % $p_x\coloneqq \Pr[\D \to x]$.
    % % % $p_x\coloneqq \Pr[\D_n \to x]$.
    % % $p_x$.
    % % In other words,
    % such that
    % $$\Pr_{x\randfrom \mathcal{D}_n}[p_x\leq \cala(x) \leq 8p_x] \geq 1 - n^{1-c/2}$$
    % % infinitely often.
    % for infinitely many $n \in \bbn$.

    Let $c > 0$.
    If there do not exist $n^{-c}$-secure distributional one-way puzzles,
    then, for any family of quantum samplable distributions $\D$,
    there is a QPT algorithm 
    % $A(x)$ 
    $\cala$
    which multiplicatively estimates 
    % % $p_x\coloneqq \Pr[\D \to x]$.
    $p_x\coloneqq \Pr[\D_n \to x]$ infinitely often.
    % where $x \in \blt^n$.
    % $p_x$.
    In other words,
    % such that
    we have
    $$\Pr_{\substack{x\randfrom \mathcal{D}_n \\ \cala}}
    [p_x\leq \cala(x) \leq 8p_x] 
    \geq 1 - n^{1-c/2}$$
    % infinitely often.
    for infinitely many $n \in \bbn$.

% 
%     Let $c > 0$ and
%     assume there does not exist a one-way puzzle.
%     % Let $\cald = \set{\cald_n}_{n \in \bbn}$ be a quantumly samplable distribution
%     Let $\cald$ be a QPT algorithm such that $\cald_n := \cald(1^n) \in \blt^n$.
%     % and let $q \geq 1$ be an arbitrary constant.
%     For $x \in \blt^n$, let 
%     % $p_x := \Pr_{x' \flws \cald_n}[x' = x]$.
%     $p_x\coloneqq \Pr[\D \to x]$.
%     There exists a QPT algorithm 
%     % $\cala$
%     $A$
%     such that, for infinitely many $n \in \bbn$, we have
%     % \bnote{is the i.o. condition necessary?}
%     \begin{equation*}
%         \Pr_{x \flws \cald_n}
%         % [\Omega(p_x) \leq \cala(x) \leq p_x]
%         [\Omega(p_x) \leq A(x) \leq p_x]
%         \geq 
%         % 1-O(1/n^q).
%         1-n^{1-c/2}.
%     \end{equation*}
\end{lemma}

Indeed, \Cref{thm:dist-owpuzz} states that, if one-way puzzles do not exist,
then $n^{-c}$-secure distributional one-way puzzles do not exist
for every $c > 0$.
In particular, setting $c=2(d+1)$ in \Cref{lemma:probest}, 
\Cref{thm:owpuzz-probest} follows.
We now prove the lemma.

\begin{proof}[Proof of \Cref{lemma:probest}]

% Without loss of generality, we will assume the output length of $\D_{n}$ is $n$.
% \bnote{An alternative way of doing that (the way done in IRS) is to let the
% sampler be an algorithm $S$ such that $S(1^n)$ samples a string in
% $\blt^n$.
% If the output length of the sampler is arbitrary, it's not entirely obvious
% how to assume it is equal to $n$ without loss of generality\ldots?
% }

Let $\mathcal{H}_n^k$ be a family of pairwise independent hash functions
with input $\{0,1\}^n$ and output $\{0,1\}^k$. 
% Let $p_x := \Pr[\cald_n \to x]$.
On input $1^n$,
% the 
define a
distributional
one-way puzzle candidate $\Samp$ 
% will behave 
as follows:
% \begin{enumerate}
%     \item Sample $k \randfrom [n]$.
%     \item Sample $h\randfrom \mathcal{H}_n^k$.
%     \item Sample $x \randfrom \D_{n}$.
%     \item Output $(k,h,h(x))$ as the puzzle and $x$ as the key.
% \end{enumerate}
\begin{algorithm}[H]
\caption{One-way puzzle candidate $\Samp$}
\begin{algorithmic}[1]
    \State \textbf{Input:} Number $n \in \bbn$ in unary ($1^n$).
    \State Sample $k \randfrom [2n]$.
    \State Sample $h\randfrom \mathcal{H}_n^k$.
    \State Sample $x \randfrom \D_{n}$.
    \State Output $(k,h,h(x))$ as the puzzle and $x$ as the key.
\end{algorithmic}
\end{algorithm}


Since $n^{-c}$-distributional one-way puzzles do not exist, there exists an
algorithm $\mathcal{O}$ which distributionally inverts $\Samp$ infinitely
often. In particular, for infinitely many $n$,
the distributions
\begin{align*}
    P_n &\coloneqq (k,h,h(x),x), \; \text{and}\\
\wt{P}_n &\coloneqq (k,h,h(x),\mathcal{O}(k,h,h(x)))
\end{align*}
satisfy
$$\Delta(P_n,\wt{P}_n) \leq n^{-c}.$$
From now on, fix $n \in \bbn$
such that the distributional inverter $\calo$ satisfies the above
inequality.
We now define the distribution $P_{k,x}$ as follows:
\begin{enumerate}
    \item Sample $h:\{0,1\}^n \to \{0,1\}^k$ a random pairwise independent
        hash function from $\calh_n^k$.
    \item Sample $x' \randfrom \D_n$ conditioned on $h(x') = h(x)$.
    \item Output $x'$.
\end{enumerate}
We first observe that, if $k$ is large, then
the probability that $P_{k,x}$ outputs $x$ is large.
Moreover, if $k$ is small,
the probability that $P_{k,x}$ outputs $x$ is smaller.
\begin{lemma}\label{claim:approx}
    If $2^{-k} \leq p_x$, then $\Pr[P_{k,x} \to x] \geq \frac{1}{2}$.
    If $2^{-k} \geq 6p_x$, then $\Pr[P_{k,x} \to x] \leq \frac{1}{4}$.
\end{lemma}

We define another distribution $\wt{P}_{k,x}$ as follows:
\begin{enumerate}
    \item Sample $h:\{0,1\}^n \to \{0,1\}^k$ a random pairwise independent
        hash function from $\calh_n^k$.
    \item Output $\mathcal{O}(k,h,h(x))$.
\end{enumerate}
We claim that this distribution approximates $P_{k,x}$ with large
probability. 
\begin{lemma}
    \label{claim:close}
    Let $d \leq \frac{c-1}{2}$. 
    With probability at least $1-n^{-d}$ over $x$, for all $k \in [2n]$,
    $$\Delta(P_{k,x},\wt{P_{k,x}}) \leq n^{-d}.$$
\end{lemma}
Crucially, the claim shows that, with large probability over
$x \flws \cald$,
the distributions $P_{k,x}$ and $\wt{P_{k,x}}$ have small statistical
distance
\emph{for all $k$}.
Moreover, note that $P_{k,x}$ is not samplable, while $\wt{P}_{k,x}$ is. 
% Thus, we can use $\wt{P}_{k,x}$ to approximate $P_{k,x}$. 
% Furthermore, we
% know that $P_{k,x}$ is very close to constant times $x$ when $2^{-k}$ is
% close to $p_x$. 
Together with \Cref{claim:approx},
this means we can approximate $p_x$
by 
% estimating $\wt{P}_{k,x}$.
sampling $\wt{P}_{k,x}$ over many values of $k$
and estimating its probability.
We formalize this idea in the following algorithm to approximate $p_x$.
% Let $t$ be some constant to be set later.
Let $t = \poly(n)$ be a large enough polynomial.

\begin{algorithm}[H]
\caption{Probability estimation algorithm $\cala$}
    \label{alg:est}
\begin{algorithmic}[1]
    \For{$k \in [2n]$}
        \For{$j \in [t]$}
            \State
            Sample $h \flws \calh_n^k$
            \State
            Let $x'_{k,j} \leftarrow \calo(k,h,h(x))$
        \EndFor
        \State
        Let $c(k) \leftarrow $ the number of $j$ such that $x'_{k,j} = x$
    \EndFor
    \State
    Let $k^*$ be the smallest $k$ such that $c(k) \geq \frac{3}{8}t$. 
    If none exists, set $k^* = 2n$.
    \label{line:test}
    \State
    Output $2^{-(k^* - 1)}$.
\end{algorithmic}
\end{algorithm}

% \begin{enumerate}
%     \item For each $k\in [2n]$.
%     \begin{enumerate}
%         \item For each $j \in [n]$
%         \begin{enumerate}
%             \item Sample $h\randfrom \mathcal{H}_n^k$
%             \item Run $\mathcal{O}(i,h,h(x)) \to x'_{k,j}$
%         \end{enumerate}
%         \item Set $c(k) = $ the number of $j$ such that $x'_{k,j} = x$
%     \end{enumerate}
%     \item Let $k^*$ be the smallest $k$ such that $c(k) \geq \frac{3}{8}t$. If none exists set $k^* = n$.
%     \item Output $2^{-(k^* - 1)}$.
% \end{enumerate}

We claim that the algorithm correctly estimates $p_x$ when
$p_x \geq 2^{-2n}$ and $x$ is such that $P_{k,x}$ and $\wt{P_{k,x}}$ are
statistically close.
Henceforth, let $d=\frac{c-1}{2}$. 
\begin{lemma}\label{claim:correctness}
    Let $x$ be such that $\Delta(P_{k,x},\wt{P}_{k,x}) \leq n^{-d}$ 
    for all $k$ and such that $p_x \geq 2^{-2n}$. 
    We claim that 
    $$\Pr[p_x \leq \cala(x) \leq 8p_x] \geq 1 - n^{-c}$$
    infinitely often.
\end{lemma}
We are now ready to conclude the proof.
First note that
\begin{equation*}
\Pr_{x\randfrom \D_n}[p_x \leq 2^{-2n}] 
\leq 
\sum_{x \in \blt^n : p_x \leq 2^{-2n}} p_x
\leq 
2^n \cdot 2^{-2n} \leq 2^{-n}. 
\end{equation*}
Furthermore,
by~\Cref{claim:close}, we have
$\Pr_{x\randfrom \D_n}[\Delta(P_{i,x},\wt{P}_{i,x})
\geq n^{-d}] \leq n^{-d}$. 
Putting this all together, we get by \Cref{claim:correctness}
that
\begin{equation*}
    \Pr_{x \flws \cald_n}[p_x \leq \cala(x) \leq 8p_x] \geq 1 - n^{-c} - n^{-d} - 2^{-n} \geq 1 -
    3n^{-d} \geq 1 - n^{1-c/2}.
\end{equation*}
\end{proof}

% This follows from setting $c$ in~\Cref{theorem:probest} to be $2(d+1)$.




==> proofsofclaims.tex <==
\subsection{Proofs of claims}

% \subsubsection{Proof of~\Cref{claim:approx}}

\begin{proof}[Proof of~\Cref{claim:approx}]
    The definitions of conditional probability and pairwise independence
    give us
    \begin{equation*}
            \Pr[P_{k,x} \to x] 
            = 
            \frac{\Pr_{h,x' \randfrom \D}[h(x') = h(x)\text{ and }x' = x]}{\Pr_{h,x' \randfrom \D}[h(x') = h(x)]}.
    \end{equation*}
    Since $x' = x$ implies $h(x') = h(x)$, the numerator simplifies to
    $\Pr_{x' \randfrom \D}[x' = x] = p_x$.
    Moreover,
    using the pairwise independence of the hash family, we obtain that
    the denominator is equal to
    \begin{align*}
        \Pr&_{h,x' \randfrom \D}[h(x') = h(x) | x' \neq x] \cdot \Pr_{x' \randfrom \D}[x' \neq x] 
        \\&+ 
        \Pr_{h,x'\randfrom \D}[h(x') = h(x) | x' = x] \cdot \Pr_{x' \randfrom \D}[x' = x]
        \\&= 
        2^{-k}(1- p_x) + p_x.
    \end{align*}
    We conclude that
    \begin{equation*}
        \Pr[P_{k,x} \to x]  = \frac{p_x}{2^{-k}(1- p_x) + p_x}.
    \end{equation*}
    
    Observe that, if $2^{-k} \leq p_x$, then since $(1-p_x) \leq 1$,
    we have
    $$\Pr[P_{k,x} \to x] \geq \frac{p_x}{p_x \cdot 1 + p_x} = \frac{1}{2}$$
    Moreover, if $2^{-k} \geq 6p_x$ and $p_x \leq \frac{1}{2}$, then since $1-p_x \geq \frac{1}{2}$,
    $$\Pr[P_{k,x} \to x] \leq \frac{p_x}{6p_x(1-p_x) + p_x} \leq \frac{p_x}{4p_x} = \frac{1}{4}$$
    Furthermore, if $p_x > \frac{1}{2}$, then $6p_x > 1$ and so we cannot have $2^{-k} \geq 6p_x$. Thus, we can ignore the second condition.
\end{proof}

% \subsubsection{Proof of~\Cref{claim:close}}

\begin{proof}[Proof of~\Cref{claim:close}]
    To ease notation, let $P = P_{k,x}$ and $\wt{P} = \wt{P_{k,x}}$.
    First, we will observe an equivalent sampling procedure for
    $P$.
    \begin{enumerate}
        \item Sample $k \randfrom [2n]$.
        \item Sample $h\randfrom \mathcal{H}_n^k$.
        \item Sample $x \randfrom \D_{n}$.
        \item Sample $x' \randfrom \D_n$ conditioned on $h(x') = h(x)$.
        \item Output $(k,h,h(x),x')$.
    \end{enumerate}
    We obtain
    % \bnote{We may want to improve this chain of equalities in the final
    % online version, but this does not seem urgent now.}
    \begin{align*}
        % \begin{split}
            \Delta&(P,\wt{P}) = \frac{1}{2}\sum_{k,h,y,x'}
            \abs{\Pr[P \to (k,h,y,x')] - \Pr[\wt{P} \to (k,h,y,x')]}
            \\&=\frac{1}{n}\sum_k \left(\frac{1}{2}\sum_{h,y,x'}
                \abs{
                \begin{aligned}
                    \frac{1}{2^{\abs{h}}}&\Pr_{x \randfrom \D}[h(x) = y]\Pr_{x \randfrom \D}[x = x' | h(x) = y]
                    \\-& 
                    \frac{1}{2^{\abs{h}}}\Pr_{x \randfrom \D}[h(x) = y]\Pr[\mathcal{O}(k,h,y) = x']
                \end{aligned}
                }
        \right)
            \\&=\E_k\left[\sum_{h,y}\left(\Pr_{x\randfrom \D}[h(x) = y]\frac{1}{2}\sum_{x'}\abs{\frac{1}{2^{|h|}}\Pr_{x\randfrom \D}[x = x' | h(x) = y] - \frac{1}{2^{|h|}}\Pr[\mathcal{O}(k,h,y) = x']}\right)\right]\\
            \\&=\E_k\left[\sum_h\E_{y\randfrom h(\mathcal{D})}\left[\frac{1}{2}\sum_{x'}\abs{\frac{1}{2^{|h|}}\Pr_{x\randfrom \D}[x = x' | h(x) = y] - \frac{1}{2^{|h|}}\Pr[\mathcal{O}(k,h,y) = x']}\right]\right]\\
            \\&=\E_k\left[\sum_h\E_{x\randfrom \D}\left[\frac{1}{2}\sum_{x'}\abs{\frac{1}{2^{|h|}}\Pr_{x''\randfrom \D}[x'' = x' | h(x'') = h(x)] - \frac{1}{2^{|h|}}\Pr[\mathcal{O}(k,h,h(x)) = x']}\right]\right]\\
            \\&\geq \E_k\left[\E_{x\randfrom \D}\left[\frac{1}{2}\sum_{x'}\abs{\sum_h\left(\frac{1}{2^{|h|}}\Pr_{x''\randfrom \D}[x'' = x' | h(x'') = h(x)] - \frac{1}{2^{|h|}}\Pr[\mathcal{O}(k,h,h(x)) = x']\right)}\right]\right]\\
            \\&= \E_k\left[\E_{x\randfrom \D}\left[\frac{1}{2}\sum_{x'}\abs{\Pr_{h,x''\randfrom \D}[x'' = x' | h(x'') = h(x)] - \Pr_h[\mathcal{O}(k,h,h(x)) = x']}\right]\right]\\
            \\&= \E_{k,x\randfrom \D}\left[\Delta(P_{k,x},\wt{P}_{k,x})\right].
        % \end{split}
    \end{align*}
    
    We briefly explain each of the equalities above.
    The first follows the definitions of $P$ and $\wt{P}$,
    using also the fact that $k$ is sampled uniformly in both
    distributions,
    and from the fact that $h$ is also sampled uniformly from a pairwise
    independent hash family.
    The second equality simply used the linearity of expectation
    and the definition of expectation. 
    The third equality again uses the definition of expectation.
    The fourth equality
    simply rewrites the previous one.
    The fifth line (and only inequality) 
    uses the triangle inequality.
    The sixth and seventh equations use the definition of expectation.



    
    Since $\Delta(P,\wt{P}) \leq n^{-c}$, the inquality above implies
    $\E_{k,x}[\Delta(P_{k,x},\wt{P}_{k,x})] \leq n^{-c}$. 
    We can then show that,
    with probability $1-n^{-d}$ over $x$, 
    it holds that $\Delta(P_{k,x},\wt{P}_{k,x}) \leq n^{-d}$
    for all $k$.
    Indeed, suppose not: then with
    probability $n^{-d}$ over $x$, there exists a $k$ such that
    $\Delta(P_{k,x},\wt{P}_{k,x}) > n^{-d}$. Thus, with probability
    $n^{-d}\cdot n^{-1}$ over $x$ and $k$, we obtain $\Delta(P_{i,x},\wt{P}_{i,x}) >
    n^{-d}$. But then $\E_{k,x}[\Delta(P_{i,x},\wt{P}_{i,x})] > n^{-2d-1}
    \geq n^{-c}$, and we reach a contradiction.
\end{proof}

% \subsubsection{Proof of~\Cref{claim:correctness}}

\begin{proof}[{Proof of~\Cref{claim:correctness}}]
    %\bnote{Where is $p_x \geq 2^{-2n}$ used?}\mnote{I'm not seeing it, and it should be in here somewhere.}


    We first show that $\cala(x) \geq p_x$ with probability at least
    $1-n^{-c}/2$.
    Note that if the test (Line~\ref{line:test} of \Cref{alg:est}) passes for some $k \leq
    \ceil{-\log p_x}$, then $\cala$ outputs $2^{-k} \geq 2^{-(\ceil{-\log p_x}
    - 1)} = 2^{\floor{\log p_x} + 1} \geq 2^{\log p_x} = p_x$.
    Thus,
    $$\Pr_{x \flws \cald_n}[\cala(x) \geq p_x] 
    % \geq \Pr[\text{test passes for some }k\leq \ceil{-\log p_x}] 
    \geq \Pr_{x \flws \cald_n}[\text{test passes for }k=\ceil{-\log p_x}].$$
    But we know that when $k = \ceil{-\log p_x}$, we have $2^{-k} \geq p_x$ and so,
    for infinitely many $n$, the probability that $\mathcal{O}(k,h,h(x)) =
    x$ for $k = \ceil{-\log p_x}$ is at least $\frac{1}{2} - n^{-d} \geq 0.49$
    by~\Cref{claim:approx} and 
    % \Cref{claim:close},
    the assumption that $\Delta(P_{k,x},\wt{P_{k,x}}) \leq n^{-d}$,
    supposing $n$ is sufficiently large.
    % and for sufficiently large
    % $n$. 
    Thus, by the Chernoff bound,
    % since for all sufficiently large $n$, $n^{-d} \leq \frac{1}{16}$, 
    we
    have 
    $$\Pr_{x \flws \cald_n}[\cala(x) \geq p_x] \geq
    1-\exp\left(-O(t)\right) \geq 1-n^{-c}/2,$$
    for infinitely many $n$, since $t = \poly(n)$.

    We now show that $\cala(x) \leq 8p_x$ with probability at least
    $1-n^{-c}/2$.
    Note that as long as the test fails for all $k \leq -\log 8p_x$, then
    $\cala(x) \leq 8p_x$. 
    But if $k \leq -\log 8p_x$, then $2^{-k} \geq 2^{-\log p_x + 3}
    \geq 6p_x$. Since $n^{-d} \leq \frac{1}{16}$ for large enough
    $n$, by the Chernoff bound, Claim~\ref{claim:approx}
    % and~\ref{claim:close},
    and the assumption,
    the
    probability that the test passes for any given $k \leq -\log 8p_x$ is
    at most $\exp(-\Omega(t))$.
    % $$\leq \exp\left(-\frac{1}{240}t\right)$$ 
    Therefore,
    by the union bound, we have that
    $$\Pr[\cala(x) \geq 8p_x] \leq
    % 2n\exp\left(-\frac{1}{240}n\right) 
    2n \cdot \exp\left(-\Omega(n)\right)
    \leq
    n^{-c}/2,$$ 
    for infinitely many $n$,
    using also the fact that $t = \poly(n)$ is a large enough polynomial.
\end{proof}


